Session-aware Information Embedding for E-commerce Product Recommendation

Most of the existing recommender systems assume that user's visiting history can be constantly recorded. However, in recent online services, the user identification may be usually unknown and only limited online user behaviors can be used. It is of great importance to model the temporal online user behaviors and conduct recommendation for the anonymous users. In this paper, we propose a list-wise deep neural network based architecture to model the limited user behaviors within each session. To train the model efficiently, we first design a session embedding method to pre-train a session representation, which incorporates different kinds of user search behaviors such as clicks and views. Based on the learnt session representation, we further propose a list-wise ranking model to generate the recommendation result for each anonymous user session. We conduct quantitative experiments on a recently published dataset from an e-commerce company. The evaluation results validate the effectiveness of the proposed method, which can outperform the state-of-the-art significantly.

==> sig-alternate-aux <==
\relax 
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{\thepage }}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces the flowchart of our solution.}}{\thepage }}
\newlabel{fig:flowchart}{{1}{\thepage }}
\citation{cockburn2003revisit}
\citation{crammer2001pranking}
\citation{shashua2002ranking}
\citation{chu2005new}
\citation{herbrich1999large}
\citation{freund2003efficient}
\citation{burges2005learning}
\citation{quoc2007learning}
\citation{cao2007learning}
\citation{burges2010ranknet}
\citation{dietterich2000ensemble}
\citation{ratsch2001soft}
\citation{friedman2001greedy}
\citation{wolpert1992stack}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces  Basic statistics of the provided dataset.}}{\thepage }}
\newlabel{tab:stat1}{{1}{\thepage }}
\@writefile{lot}{\contentsline {table}{\numberline {2}{\ignorespaces  User statistics of the provided dataset.}}{\thepage }}
\newlabel{tab:stat2}{{2}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {2}Dataset Overview}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {3}Related Work}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1}Learning to rank}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2}Ensemble learning}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {4}Feature Extraction}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.1}Statistic Features}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.1.1}global statistic features}{\thepage }}
\citation{robertson2009probabilistic}
\newlabel{equ:1}{{1}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.1.2}Time-based statistic features}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2}Query-Item Features}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.2.1}Category-based token features}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {4.2.2}Cross token features}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3}Session features}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {5}Model Framework}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.1}Model Selection}{\thepage }}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces deep match model.}}{\thepage }}
\newlabel{fig:dmm}{{2}{\thepage }}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces the framework of query full.}}{\thepage }}
\newlabel{fig:queryfull}{{3}{\thepage }}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2}Ensemble Modeling}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {5.2.1}Query Full}{\thepage }}
\@writefile{toc}{\contentsline {subsubsection}{\numberline {5.2.2}Query Less}{\thepage }}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces the framework of query less.}}{\thepage }}
\newlabel{fig:queryless}{{4}{\thepage }}
\@writefile{lot}{\contentsline {table}{\numberline {3}{\ignorespaces  Validation results of different models in our solution.}}{\thepage }}
\newlabel{tab:1}{{3}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {6}Results}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {7}Conclusions}{\thepage }}
\bibstyle{abbrv}
\bibdata{sigproc}
\bibcite{burges2005learning}{1}
\bibcite{burges2010ranknet}{2}
\bibcite{cao2007learning}{3}
\bibcite{chu2005new}{4}
\bibcite{crammer2001pranking}{5}
\bibcite{dietterich2000ensemble}{6}
\bibcite{freund2003efficient}{7}
\bibcite{friedman2001greedy}{8}
\bibcite{herbrich1999large}{9}
\bibcite{quoc2007learning}{10}
\bibcite{ratsch2001soft}{11}
\bibcite{robertson2009probabilistic}{12}
\bibcite{shashua2002ranking}{13}
\bibcite{wolpert1992stack}{14}
\@writefile{toc}{\contentsline {section}{\numberline {8}Acknowledgments}{\thepage }}
\@writefile{toc}{\contentsline {section}{\numberline {9}References}{\thepage }}

